RKKY in half-filled bipartite lattices: graphene as an example

We first present a simple proof that for any bipartite lattice at half filling the RKKY interaction is antiferromagnetic between impurities on opposite (i.e., A and B) sublattices and is ferromagnetic between impurities on the same sublattices. This result is valid on all length scales. We then focus on the honeycomb lattice and examine the theorem in the long distance limit by performing the low energy calculation using Dirac electrons. To find the universal (cutoff free) result we perform the calculation in smooth cutoff schemes, as we show that the calculation based on a sharp cutoff leads to wrong results. We also find the long distance behavior of the RKKY interaction between "plaquette" impurities in both coherent and incoherent regimes.

==> feynmf.1 <==
.\" Automatically generated by Pod::Man v1.37, Pod::Parser v1.14
.\"
.\" Standard preamble:
.\" ========================================================================
.de Sh \" Subsection heading
.br
.if t .Sp
.ne 5
.PP
\fB\\$1\fR
.PP
..
.de Sp \" Vertical space (when we can't use .PP)
.if t .sp .5v
.if n .sp
..
.de Vb \" Begin verbatim text
.ft CW
.nf
.ne \\$1
..
.de Ve \" End verbatim text
.ft R
.fi
..
.\" Set up some character translations and predefined strings.  \*(-- will
.\" give an unbreakable dash, \*(PI will give pi, \*(L" will give a left
.\" double quote, and \*(R" will give a right double quote.  | will give a
.\" real vertical bar.  \*(C+ will give a nicer C++.  Capital omega is used to
.\" do unbreakable dashes and therefore won't be available.  \*(C` and \*(C'
.\" expand to `' in nroff, nothing in troff, for use with C<>.
.tr \(*W-|\(bv\*(Tr
.ds C+ C\v'-.1v'\h'-1p'\s-2+\h'-1p'+\s0\v'.1v'\h'-1p'
.ie n \{\
.    ds -- \(*W-
.    ds PI pi
.    if (\n(.H=4u)&(1m=24u) .ds -- \(*W\h'-12u'\(*W\h'-12u'-\" diablo 10 pitch
.    if (\n(.H=4u)&(1m=20u) .ds -- \(*W\h'-12u'\(*W\h'-8u'-\"  diablo 12 pitch
.    ds L" ""
.    ds R" ""
.    ds C` ""
.    ds C' ""
'br\}
.el\{\
.    ds -- \|\(em\|
.    ds PI \(*p
.    ds L" ``
.    ds R" ''
'br\}
.\"
.\" If the F register is turned on, we'll generate index entries on stderr for
.\" titles (.TH), headers (.SH), subsections (.Sh), items (.Ip), and index
.\" entries marked with X<> in POD.  Of course, you'll have to process the
.\" output yourself in some meaningful fashion.
.if \nF \{\
.    de IX
.    tm Index:\\$1\t\\n%\t"\\$2"
..
.    nr % 0
.    rr F
.\}
.\"
.\" For nroff, turn off justification.  Always turn off hyphenation; it makes
.\" way too many mistakes in technical documents.
.hy 0
.if n .na
.\"
.\" Accent mark definitions (@(#)ms.acc 1.5 88/02/08 SMI; from UCB 4.2).
.\" Fear.  Run.  Save yourself.  No user-serviceable parts.
.    \" fudge factors for nroff and troff
.if n \{\
.    ds #H 0
.    ds #V .8m
.    ds #F .3m
.    ds #[ \f1
.    ds #] \fP
.\}
.if t \{\
.    ds #H ((1u-(\\\\n(.fu%2u))*.13m)
.    ds #V .6m
.    ds #F 0
.    ds #[ \&
.    ds #] \&
.\}
.    \" simple accents for nroff and troff
.if n \{\
.    ds ' \&
.    ds ` \&
.    ds ^ \&
.    ds , \&
.    ds ~ ~
.    ds /
.\}
.if t \{\
.    ds ' \\k:\h'-(\\n(.wu*8/10-\*(#H)'\'\h"|\\n:u"
.    ds ` \\k:\h'-(\\n(.wu*8/10-\*(#H)'\`\h'|\\n:u'
.    ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'^\h'|\\n:u'
.    ds , \\k:\h'-(\\n(.wu*8/10)',\h'|\\n:u'
.    ds ~ \\k:\h'-(\\n(.wu-\*(#H-.1m)'~\h'|\\n:u'
.    ds / \\k:\h'-(\\n(.wu*8/10-\*(#H)'\z\(sl\h'|\\n:u'
.\}
.    \" troff and (daisy-wheel) nroff accents
.ds : \\k:\h'-(\\n(.wu*8/10-\*(#H+.1m+\*(#F)'\v'-\*(#V'\z.\h'.2m+\*(#F'.\h'|\\n:u'\v'\*(#V'
.ds 8 \h'\*(#H'\(*b\h'-\*(#H'
.ds o \\k:\h'-(\\n(.wu+\w'\(de'u-\*(#H)/2u'\v'-.3n'\*(#[\z\(de\v'.3n'\h'|\\n:u'\*(#]
.ds d- \h'\*(#H'\(pd\h'-\w'~'u'\v'-.25m'\f2\(hy\fP\v'.25m'\h'-\*(#H'
.ds D- D\\k:\h'-\w'D'u'\v'-.11m'\z\(hy\v'.11m'\h'|\\n:u'
.ds th \*(#[\v'.3m'\s+1I\s-1\v'-.3m'\h'-(\w'I'u*2/3)'\s-1o\s+1\*(#]
.ds Th \*(#[\s+2I\s-2\h'-\w'I'u*3/5'\v'-.3m'o\v'.3m'\*(#]
.ds ae a\h'-(\w'a'u*4/10)'e
.ds Ae A\h'-(\w'A'u*4/10)'E
.    \" corrections for vroff
.if v .ds ~ \\k:\h'-(\\n(.wu*9/10-\*(#H)'\s-2\u~\d\s+2\h'|\\n:u'
.if v .ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'\v'-.4m'^\v'.4m'\h'|\\n:u'
.    \" for low resolution devices (crt and lpr)
.if \n(.H>23 .if \n(.V>19 \
\{\
.    ds : e
.    ds 8 ss
.    ds o a
.    ds d- d\h'-1'\(ga
.    ds D- D\h'-1'\(hy
.    ds th \o'bp'
.    ds Th \o'LP'
.    ds ae ae
.    ds Ae AE
.\}
.rm #[ #] #H #V #F C
.\" ========================================================================
.\"
.IX Title "FEYNMF 1"
.TH FEYNMF 1 "1996-12-02" "FeynMF Version 1.08" "Contributed LaTeX Utilities"
.SH "NAME"
\&\fBfeynmf\fR \- Process \fBLaTeX\fR files using \fBFeynMF\fR
.SH "SYNOPSIS"
.IX Header "SYNOPSIS"
\&\fBfeynmf\fR [\fB\-hvqncfT\fR] [\fB\-t\fR \fItfm\fR [\fB\-t\fR \fItfm\fR ...]] [\fB\-m\fR \fImode\fR]
       \fIfile\fR [\fIfile\fR ...]
.PP
\&\fBfeynmf\fR [\fB\-\-help\fR] [\fB\-\-version\fR] [\fB\-\-quiet\fR] [\fB\-\-noexec\fR] [\fB\-\-clean\fR]
       [\fB\-\-force\fR] [\fB\-\-notfm\fR] [\fB\-\-tfm\fR \fItfm\fR [\fB\-\-tfm\fR \fItfm\fR ...]]
       [\fB\-\-mode\fR \fImode\fR] \fIfile\fR [\fIfile\fR ...]
.SH "DESCRIPTION"
.IX Header "DESCRIPTION"
The most complicated part of using the \fBFeynMF\fR style appears to be the
proper invocation of \fBMetafont\fR.  The \fBfeynmf\fR script provides a
convenient front end and will automagically invoke \fBMetafont\fR with the
proper mode and magnifincation.  It will also avoid cluttering system font
directories and offers an option to clean them.
.SH "OPTIONS"
.IX Header "OPTIONS"
.IP "\fB\-h\fR, \fB\-\-help\fR" 4
.IX Item "-h, --help"
Print a short help text.
.IP "\fB\-v\fR, \fB\-\-version\fR" 4
.IX Item "-v, --version"
Print the version of \fBfeynmf\fR.
.IP "\fB\-q\fR, \fB\-\-quiet\fR" 4
.IX Item "-q, --quiet"
Don't echo the commands being executed.
.IP "\fB\-n\fR, \fB\-\-noexec\fR" 4
.IX Item "-n, --noexec"
Don't execute \fBLaTeX\fR or \fBMetafont\fR.
.IP "\fB\-c\fR, \fB\-\-clean\fR" 4
.IX Item "-c, --clean"
Offer to delete font files that have accidentally been placed in a
system directory by the \fBMakeTeXTFM\fR and \fBMakeTeXPK\fR scripts (these
scripts are run by \fBtex\fR (and \fBlatex\fR) in the background).  This
option has only been tested with recent versions of \s-1UNIX\s0 TeX.
.IP "\fB\-f\fR, \fB\-\-force\fR" 4
.IX Item "-f, --force"
Don't ask any questions.
.IP "\fB\-T\fR, \fB\-\-notfm\fR" 4
.IX Item "-T, --notfm"
Don't try to prepare fake \f(CW\*(C`.tfm\*(C'\fR files for the first run.
.IP "\fB\-t\fR, \fB\-\-tfm\fR \fItfm\fR" 4
.IX Item "-t, --tfm tfm"
Don't try guess the names of the \f(CW\*(C`.tfm\*(C'\fR files to fake for
the first run and use the given name(s) instead.  This option
can be useful if our incomplete parsing of the LaTeX input
files fails.
.IP "\-\fBm\fR \fImode\fR, \fB\-\-mode\fR \fImode\fR" 4
.IX Item "-m mode, --mode mode"
Select the \s-1METAFONT\s0 mode \fImode\fR.  The default is guessed or
\&\f(CW\*(C`localfont\*(C'\fR if the guess fails.
.IP "\fIfile\fR" 4
.IX Item "file"
Main \fBLaTeX\fR input files.
.IP "\fIfile\fR ..." 4
.IX Item "file ..."
Other LaTeX input files that are included by the main file.
.SH "AUTHOR"
.IX Header "AUTHOR"
Thorsten Ohl <Thorsten.Ohl@Physik.TH\-Darmstadt.de>
.SH "BUGS"
.IX Header "BUGS"
The preparation of \f(CW\*(C`.tfm\*(C'\fR files is not foolproof yet, because we can
parse \fBTeX\fR files only superficially.
.PP
This script has only been tested for recent \fBteTeX\fR distributions
of \s-1UNIX\s0 \fBTeX\fR, though it will probably work with other versions of
\&\s-1UNIX\s0 \fBTeX\fR.  The author will be grateful for portability suggestions,
even concerning \fBBorg\fR operating systems, for the benefit of those users
that are forced to live with \s-1DOS\s0 or Windows.

